Rzk: a Proof Assistant for Synthetic $\infty$-Categories

Homotopy type theory (HoTT) is a type theory that allows for synthetic reasoning about $\infty$-groupoids. Several proof assistants (such as Rocq and Agda) implement variants of HoTT. Directed type theory is a type theory for synthetic reasoning about $\infty$-categories, where morphisms (or paths) of dimension 1 are not necessarily invertible. Among the proposals for directed type theory, the most developed is Riehl and Shulman's simplicial type theory (RSTT), based on simplicial shapes such as directed intervals and triangles. We present Rzk, a proof assistant implementing (a refinement of) RSTT for synthetic reasoning about $\infty$-categories. Specifically, the type theory implemented by Rzk is a computational variant of RSTT adjusted to make type checking practical. We define a translation from RSTT to Rzk and prove that it is sensible: every RSTT proof translates to an Rzk proof (faithfulness), and Rzk proves nothing new about RSTT types (conservativity). We also give a tutorial introduction to proving in Rzk, and describe its implementation, including the type-checking algorithm and the automated prover for the logic of shapes.

==> figures/rstt-rzk-translation.tex <==
\begin{figure*}
  \centering
  \begin{tikzpicture}[
      box/.style={draw, rounded corners, align=center, inner sep=6pt, font=\small},
      lbl/.style={font=\scriptsize\itshape, align=center},
      arr/.style={-{Stealth}}
    ]
    \node[box] (inner) at (0, 0)
      {\RSTT{} statement\\[2pt]
       fixed $\tp{\psi}, \tp{\phi}$;\quad side condition $\pt{t} : \cube{I} \mid \tp{\phi} \vdash \tp{\psi}$\\[2pt]
       $\cube{\Xi} \mid \tp{\Phi} \mid \ty{\Gamma} \vdash J$};
    \node[lbl] (quant) at (0, 1.2)
      {$\forall\; \cube{I} : \cube{\cubeU},\;
        \tp{\psi}, \tp{\phi} : \cube{I} \to \tp{\mathsf{TOPE}}$ \;with\; $\tp{\phi} \vdash \tp{\psi}$};
    \node[box, fit=(quant)(inner), inner sep=9pt, label={[font=\small]above:\RSTT{} $+$ meta-theoretic parameter layer (\RSTTMTPL{})}] (outer) {};
    \node[box, anchor=west] (rzk) at ([xshift=2.4cm]outer.east)
      {\dRzk{}: one schematic \texttt{\#def}\\[2pt]
       $\cube{\Xi} \mid \tp{\Phi} \mid \ty{\Gamma} \vdash M : \ty{T}$};
    \draw[arr] (outer.east) -- (rzk.west)
      node[midway, above, font=\small] {$\tau$};
  \end{tikzpicture}
  \caption{Relating \Rzk{} to \RSTT{}. An \RSTT{} statement (left box) is about fixed topes
  $\tp{\psi}, \tp{\phi}$ and carries entailment side conditions, here
  $\pt{t} : \cube{I} \mid \tp{\phi} \vdash \tp{\psi}$, proved in the meta-theory. The
  meta-theoretic parameter layer wrapping it makes that meta-level quantification explicit: the cube
  and the topes become parameters, and each inclusion $\tp{\phi} \vdash \tp{\psi}$ becomes a parameter
  domain, which \Rzk{} records as a tope family $\tp{\phi} : \tp{\psi} \to \tp{\mathsf{TOPE}}$
  (\cref{sec:tope-params}). The translation $\tau$ keeps the layer in place, and \Rzk{} renders the
  translated statement as a single \emph{schematic} definition over first-class parameters. Conservativity
  (\cref{thm:conservativity}) is the converse, back-translating the \Rzk{} definition to an \RSTT{}
  statement schematic over the layer.}
  \label{fig:rstt-rzk-translation}
\end{figure*}


==> figures/tope-families.tex <==
\subsection{Shapes and Subshapes}

\RSTT{} defines shapes as a shorthand for a pair of a cube and a tope, restricting that cube.

==> preamble.tex <==
\usepackage[capitalize]{cleveref}
\usepackage{aliascnt}
\makeatletter
\newcommand{\rzkpaper@newthm}[3]{%
  \theoremstyle{#1}%
  \newaliascnt{#2}{theorem}%
  \newtheorem{#2}[#2]{#3}%
  \aliascntresetthe{#2}%
}
\theoremstyle{acmplain}
\newtheorem{theorem}{Theorem}[section]
\rzkpaper@newthm{acmplain}{conjecture}{Conjecture}
\rzkpaper@newthm{acmplain}{proposition}{Proposition}
\rzkpaper@newthm{acmplain}{lemma}{Lemma}
\rzkpaper@newthm{acmplain}{corollary}{Corollary}
\rzkpaper@newthm{acmdefinition}{example}{Example}
\rzkpaper@newthm{acmdefinition}{definition}{Definition}
\rzkpaper@newthm{acmdefinition}{remark}{Remark}
\makeatother
\crefname{conjecture}{Conjecture}{Conjectures}
\crefname{proposition}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{example}{Example}{Examples}
\crefname{definition}{Definition}{Definitions}
\crefname{remark}{Remark}{Remarks}
\crefname{appendix}{Appendix}{Appendices}
\crefname{subappendix}{Appendix}{Appendices}
\crefformat{section}{\S#2#1#3}
\Crefformat{section}{\S#2#1#3}
\crefrangeformat{section}{\S\S#3#1#4--#5#2#6}
\Crefrangeformat{section}{\S\S#3#1#4--#5#2#6}
\crefmultiformat{section}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\Crefmultiformat{section}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}
\usepackage{tikz}
\usetikzlibrary{arrows.meta, fit, positioning}
\usepackage{subcaption}
\usepackage{bussproofs}
\usepackage{xspace}

\usepackage[inline]{enumitem}

\usepackage{bbm} %
\usepackage{multirow} %
\usepackage{bigdelim} %

\usepackage[unicode]{rzk}   %

\usepackage{minted}                   %
\setminted{fontsize=\small,texcomments}
\usemintedstyle{xcode}                %
\newmintinline[code]{agda}{bgcolor=gray!10}  %
\newcommand{\rzkinput}[2][]{\inputminted[firstline=2,frame=lines,#1]{rzk}{#2}}

\newcommand{\extann}[3]{#1 \left\rvert \phantom{}^{#2}_{#3} \right.}
\newcommand{\exttype}[4]{\left\langle \prod\nolimits_{#1} #2 \middle\vert \phantom{}^{#3}_{#4} \right\rangle}
\newcommand{\exttypefun}[4]{\left\langle {#1} \to {#2} \middle\vert \phantom{}^{#3}_{#4} \right\rangle}

\newcommand{\checked}[1]{{\color{OliveGreen}#1}}
\newcommand{\unchecked}[1]{{\color{gray}#1}}      %
\newcommand{\cube}[1]{{\color{Brown}#1}}          %
\newcommand{\pt}[1]{{\color{BurntOrange}#1}}      %
\newcommand{\tp}[1]{{\color{RoyalBlue}#1}}        %
\newcommand{\ty}[1]{{\color{OliveGreen}#1}}       %
\newcommand{\cubeU}{\mathsf{Cube}}
\newcommand{\topeU}{\mathsf{Tope}}
\newcommand{\typeU}{\mathsf{Type}}
\newcommand{\refl}[2]{\mathsf{refl}_{#1}\left(#2\right)}
\newcommand{\subtype}{\mathrel{<:}}

\DeclareMathOperator{\meq}{\stackrel{?}{=}}
\DeclareMathOperator{\shape}{\mathsf{shape}}

\newcommand{\metavar}[2]{{\normalfont\color{RoyalBlue}{\textsc{#1}{#2}}}}
\newcommand{\type}[1]{{\color{OliveGreen}{#1}}}  %
\newcommand{\con}[1]{{\color{blue}{\mathsf{#1}}}}
\newcommand{\metasubst}[1]{{\color{Plum}{#1}}}
\newcommand{\bnfalt}[2]{{\mathop{\phantom{\langle,}#1\phantom{,\rangle}}_{\smaller\color{gray}\text{#2}}}}

\newcommand{\defcon}{{\con{F}}}
\newcommand{\mm}{{\metavar{m}{}}}
\newcommand{\app}{{\con{app}}}
\newcommand{\abs}{{\con{abs}}}
\newcommand{\subst}{{\con{subst}}}
\newcommand{\named}{{\con{named}}}
\newcommand{\ord}{{\mathsf{ord}}}

\newcommand{\systemname}[1]{\textsf{#1}\xspace}
\newcommand{\Rzk}{\systemname{Rzk}}
\newcommand{\Coq}{\systemname{Rocq}}
\newcommand{\Agda}{\systemname{Agda}}
\newcommand{\Lean}{\systemname{Lean}}
\newcommand{\Arend}{\systemname{Arend}}
\newcommand{\sHoTT}{\systemname{sHoTT}}
\newcommand{\RedPRL}{\texttt{\textcolor{red}{Red}PRL}\xspace}
\newcommand{\redtt}{\texttt{\textcolor{red}{red}tt}\xspace}
\newcommand{\cooltt}{\texttt{\textcolor{blue}{cool}tt}\xspace}

\newcommand{\declRzk}{declarative \Rzk}
\newcommand{\dRzk}{\systemname{d\Rzk}}
\newcommand{\DeclRzk}{Declarative \Rzk}
\newcommand{\algRzk}{algorithmic \Rzk}
\newcommand{\aRzk}{\systemname{a\Rzk}}
\newcommand{\AlgRzk}{Algorithmic \Rzk}

\newcommand{\RSTT}{\systemname{RSTT}}
\newcommand{\RSTTMTPL}{\systemname{\MTPL + \RSTT}}
\newcommand{\MTPL}{\systemname{MPL}}



\newcommand{\Id}[3][]{\ensuremath{#2 =_{#1}#3}}




\def\UseOption{final}  %
\usepackage[draft]{optional}

\newif\ifanonsubmission
\anonsubmissionfalse   %
\newcommand{\implref}[2]{\ifanonsubmission#2\else\href{#1}{#2}\fi}
\newcommand{\rzksrcbase}{https://github.com/rzk-lang/rzk/blob/3b48d753958d63f25aa35f6207a876cdc53f0255/rzk/src/Rzk/TypeCheck.hs}
\newcommand{\srcref}[2]{\ifanonsubmission
  \shortstack{#2\\[-1pt]{\scriptsize\ttfamily #1}}%
  \else\href{\rzksrcbase\##1}{#2}\fi}
\newcommand{\srcrefinline}[2]{\ifanonsubmission#2\,{\scriptsize\ttfamily[#1]}\else\href{\rzksrcbase\##1}{#2}\fi}
\newcommand{\anonurlnote}[1]{\ifanonsubmission\else\footnote{\url{#1}}\fi}
\newcommand{\anonfootnote}[1]{\ifanonsubmission\else\footnote{#1}\fi}

\newif\ifarxiv
\arxivtrue
\newcommand{\suppmat}{\ifarxiv the ancillary files accompanying this paper\else the supplementary material\fi}
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}%

\newcommand{\plan}[1]{}
\newcommand{\NK}[1]{}
\newcommand{\BA}[1]{}
\opt{draft}{
  \renewcommand{\plan}[1]{{\color{blue}{#1}}\PackageWarning{TODO}{Plan: #1}}
  \renewcommand{\NK}[1]{\todo[color=green!30]{NK: #1}\PackageWarning{TODO}{NK: #1}}
  \renewcommand{\BA}[1]{\todo[color=orange!30]{BA: #1} \PackageWarning{TODO}{BA: #1}}
}




\newif\ifsplitappendix
\splitappendixfalse
\InputIfFileExists{submission-split}{}{}


==> sections/automated-tope-logic.tex <==
\section{Automated reasoning for tope logic}
\label{sec:automated-tope-logic-draft}

In this section, we specify the implementation for full automation
of reasoning in tope logic.




\plan{Background on automated reasoning.}

\plan{Explain the sequent-based proof search implemented in \Rzk{}.}

\plan{Give examples.}

\plan{Note that real world formalizations~\cite{KudasovRiehlWeinberger2024} have relatively small problems, which are solved fast with a naïve implementation.}

\plan{Conclude with future work?}


==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\subsection{Typechecking}

\plan{A note on the typechecking context.}

\plan{Representation of checked declarations.}

\plan{(First-order?) unification implementation}

\plan{Bidirectional type checking}

\subsection{Online Playground}

\plan{Mention GHCJS and CodeMirror setup for online playground. Thank Danila Danko for help with recent versions.}

\subsection{Language Server}

\plan{Mention the current state, challenges, and future work. Thank Abdelrahman Abounegm for the VS Code extension. Reference \url{https://www.system-informatics.ru/en/article/330}.}


==> sections/primer-on-quasicats.tex <==
\section{A Primer on Quasicategories}
\label{sec:quasicats}

